Artificial Intelligence for the Electron Ion Collider (AI4EIC)

The Electron-Ion Collider (EIC), a state-of-the-art facility for studying the strong force, is expected to begin commissioning its first experiments in 2028. This is an opportune time for artificial intelligence (AI) to be included from the start at this facility and in all phases that lead up to the experiments. The second annual workshop organized by the AI4EIC working group, which recently took place, centered on exploring all current and prospective application areas of AI for the EIC. This workshop is not only beneficial for the EIC, but also provides valuable insights for the newly established ePIC collaboration at EIC. This paper summarizes the different activities and R&D projects covered across the sessions of the workshop and provides an overview of the goals, approaches and strategies regarding AI/ML in the EIC community, as well as cutting-edge techniques currently studied in other experiments.

==> alphabetical_authorlist.tex <==
%-------------------------------------%
%--------------- README --------------%
%-------------------------------------%

% The paper will be co-authored by all the participants in the workshop.
% Sections will be first drafted by Conveners. 
% Conveners should reach out to the Invited Speakers if information on their talks is needed, and invite them to provide feedback on the session and co-author the paper.
% The final draft will be circulated among all the participants for feedback.
% Participants will have the possibility to opt-in (opt-out?). 

% Live Document https://docs.google.com/document/d/13BWnq_ywTYs__2zA0beeDob8pcuiiBiVqXNk33Kk8LY/edit 

%\author[]{\textbf{The AI4EIC workshop participants (in progress)}}

% the full authorlist will be in alphabetical order; conveners, speakers, hackathon will be specified.

%\affil*[\dagger] Convener
%\affil*[\ddagger] Invited speaker


%\begin{comment}
%\author*[1,2]{\fnm{First} \sur{Author}}\email{iauthor@gmail.com}




% conveners
\author[7]{\fnm{C.} \sur{Allaire}}
\equalspeak{Invited speaker}
\author[8]{\fnm{R.} \sur{Ammendola}}
\equalspeak{Invited speaker}
\author[1]{\fnm{E.-C.} \sur{Aschenauer}}
\equalspeak{Invited speaker}
\author[4]{\fnm{M.} \sur{Balandat}}
\equalspeak{Invited speaker}%tutorial
\author[29]{\fnm{M.} \sur{Battaglieri}}
\equalconv{Convener}
\author[30,36]{\fnm{J.} \sur{Bernauer}}
\equalconv{Convener}
\author[10]{\fnm{M.} \sur{Bond\`i}}
\equalspeak{Invited speaker}
\author[11,63]{\fnm{N.} \sur{Branson}}
\equalspeak{Invited speaker}
\author[2]{\fnm{T.} \sur{Britton}}
\equalspeak{Invited speaker}
\author[12]{\fnm{A.} \sur{Butter}}
\equalspeak{Invited speaker}
\author[40]{\fnm{I.} \sur{Chahrour}}
\author[2]{\fnm{P.} \sur{Chatagnon}}
\author[31]{\fnm{E.} \sur{Cisbani}}
\equalconv{Convener}
\author[55]{\fnm{E. W.} \sur{Cline}}
\author[28]{\fnm{S.} \sur{Dash}}
\equalconv{Convener}
\author[3]{\fnm{C.} \sur{Dean}}
\equalspeak{Invited speaker}
\author[13]{\fnm{W.} \sur{Deconinck}}
\equalconv{Convener}
\author[30,41]{\fnm{A.} \sur{Deshpande}}
\author[2]{\fnm{M.} \sur{Diefenthaler}}
\equalconv{Convener}
\equalspeak{Invited Speaker}
\author[2]{\fnm{R.} \sur{Ent}}
\equalspeak{Invited speaker}
\corrauthor[2,5]{\fnm{C.} \sur{Fanelli}}
\equalhack{Hackathon Organizer}
\equaltut{Editor}
\equalcorr{Corresponding Author}
\author[54]{\fnm{M.} \sur{Finger}}
\author[54]{\fnm{M.} \sur{Finger, Jr.}}
\author[14]{\fnm{E.} \sur{Fol}}
\equalspeak{Invited speaker}
\author[2]{\fnm{S.} \sur{Furletov}}
\equalspeak{Invited speaker}
\author[1]{\fnm{Y.} \sur{Gao}}
\author[5,25]{\fnm{J.} \sur{Giroux}}
\equalspeak{Invited speaker}
\equalhack{Hackathon}
\author[17]{\fnm{N. C.} \sur{Gunawardhana Waduge}}
\author[60,61]{\fnm{R.} \sur{Harish}}
\author[13,46]{\fnm{O.} \sur{Hassan}}
\author[60]{\fnm{P. L.} \sur{Hegde}}
\author[56]{\fnm{R. J.} \sur{Hern\'andez-Pinto}}
\author[35]{\fnm{A.} \sur{Hiller Blin}}
\equalspeak{Invited speaker}
\author[32]{\fnm{T.} \sur{Horn}}
\equaltut{Editor}
\author[1]{\fnm{J.} \sur{Huang}}
\equalspeak{Invited speaker} %also panelist
\author[57,2]{\fnm{D.} \sur{Jayakodige}}
\author[15]{\fnm{B.} \sur{Joo}}
\equalspeak{Invited speaker}
\author[25]{\fnm{M.} \sur{Junaid}}
\author[51]{\fnm{P.} \sur{Karande}}
\author[39]{\fnm{B.} \sur{Kriesten}}
%\equalspeak{Invited speaker}
\author[16]{\fnm{R.} \sur{Kunnawalkam Elayavalli}}
\equalspeak{Invited speaker}
\author[1]{\fnm{M.} \sur{Lin}}
\author[15]{\fnm{F.} \sur{Liu}}
\equalspeak{Invited speaker}
\author[17]{\fnm{S.} \sur{Liuti}}
\equalspeak{Invited speaker}
\author[18]{\fnm{G.} \sur{Matousek}}
\author[18]{\fnm{M.} \sur{McEneaney}}
\equalspeak{Invited speaker}
\author[2]{\fnm{D.} \sur{McSpadden}}
%\equalspeak{Invited speaker}%tutorial
\equalhack{Hackathon}
\author[19]{\fnm{T.} \sur{Menzo}}
\equalspeak{Invited speaker}
\author[20]{\fnm{T.} \sur{Miceli}}
\equalspeak{Invited speaker}%panelist
\author[21]{\fnm{V.} \sur{Mikuni}}
\equalspeak{Invited speaker}%tutorial
\author[33]{\fnm{R.} \sur{Montgomery}}
\equalconv{Convener}
\author[21]{\fnm{B.} \sur{Nachman}}
\equalconv{Convener}
\equalspeak{Invited Speaker}
\author[47]{\fnm{R. R.} \sur{Nair}}
\author[5]{\fnm{J.} \sur{Niestroy}}
\author[56]{\fnm{S. A.} \sur{Ochoa Oregon}}
\author[49]{\fnm{J.} \sur{Oleniacz}} 
\author[1]{\fnm{J. D.} \sur{Osborn}}
\equalconv{Convener}
\author[42]{\fnm{C.} \sur{Paudel}}
\author[18]{\fnm{C.} \sur{Pecar}}
\equalspeak{Invited speaker}
\author[22]{\fnm{C.} \sur{Peng}}
\equalspeak{Invited speaker}
\author[20]{\fnm{G. N.} \sur{Perdue}}
\equalconv{Convener}
\author[23,2]{\fnm{W.} \sur{Phelps}}
\equalspeak{Invited speaker}
\author[1]{\fnm{M. L.} \sur{Purschke}}
\author[2]{\fnm{K.} \sur{Rajput}}
\equalspeak{Invited speaker}%tutorial
\equalhack{Hackathon}
\author[21]{\fnm{Y.} \sur{Ren}}
\equalconv{Convener}
\equalspeak{Invited speaker}%tutorial
\author[56]{\fnm{D. F.} \sur{Renteria-Estrada}}
\author[62]{\fnm{D.} \sur{Richford}}
\author[58,59]{\fnm{B. J.} \sur{Roy}}
\author[43]{\fnm{D.} \sur{Roy}}
\author[2]{\fnm{N.} \sur{Sato}}
\equalspeak{Invited speaker}
\author[2,38]{\fnm{T.} \sur{Satogata}}
\equalspeak{Invited speaker}
\author[44,45]{\fnm{G.} \sur{Sborlini}}
\author[2]{\fnm{M.} \sur{Schram}}
\equalconv{Convener}
\author[24]{\fnm{D.} \sur{Shih}}
\equalspeak{Invited speaker}
\author[52]{\fnm{J.} \sur{Singh}}
\author[41,64]{\fnm{R.} \sur{Singh}}
\author[9]{\fnm{A.} \sur{Siodmok}} %A. Siodmok
\equalspeak{Invited speaker}
\author[5]{\fnm{P.} \sur{Stone}}
\author[5]{\fnm{J.} \sur{Stevens}}
\equalconv{Convener}
\author[5]{\fnm{L.} \sur{Suarez}}
\author[25]{\fnm{K.} \sur{Suresh}}
\equalhack{Hackathon}
\author[48]{\fnm{A.-N.} \sur{Tawfik}}
\author[21]{\fnm{F.} \sur{Torales Acosta}}
\equalspeak{Invited speaker}%tutorial
\author[20]{\fnm{N.} \sur{Tran}}
\equalspeak{Invited speaker}
\author[32]{\fnm{R.} \sur{Trotta}}
\author[50]{\fnm{F. J.} \sur{Twagirayezu}}
\author[33]{\fnm{R.} \sur{Tyson}}
\author[26]{\fnm{S.} \sur{Volkova}}
\equalspeak{Invited speaker}
\author[2,18]{\fnm{A.} \sur{Vossen}}
\equalconv{Hackathon}
\author[5]{\fnm{E.} \sur{Walter}}
\equalhack{Hackathon Organizer}
\author[27]{\fnm{D.} \sur{Whiteson}}
\equalspeak{Invited speaker}
\author[3]{\fnm{M.} \sur{Williams}}
\equalspeak{Invited speaker}%panelist
\author[13]{\fnm{S.} \sur{Wu}}
\author[53]{\fnm{N.} \sur{ Zachariou}}
\author[34,37]{\fnm{P.} \sur{Zurita}}
\equalconv{Convener}

\affil[1]{\orgname{Brookhaven National Lab}, \orgaddress{\city{Upton}, \state{NY}, \postcode{11973}, \country{USA}}}
\affil[2]{\orgname{Jefferson Lab}, \orgaddress{\city{Newport News}, \state{VA}, \postcode{23606}, \country{USA}}}
\affil[3]{\orgname{Massachusetts Institute of Technology}, \orgaddress{\city{Cambridge}, \postcode{02139}, \state{MA}, \country{USA}}}
\affil[4]{\orgname{Meta}, \orgaddress{\city{Menlo Park}, \state{CA}, \postcode{94025}, \country{USA}}}
\affil[5]{\orgname{William \& Mary}, \orgaddress{\city{Williamsburg}, \state{VA}, \postcode{23185}, \country{USA}}}
\affil[6]{\orgname{University of California}, \orgdiv{Berkeley Institute for Data Science}, \orgaddress{\city{Berkeley},  \state{CA}, \postcode{94720}, \country{USA}}}
\affil[7]{\orgname{Université Paris-Saclay}, \orgdiv{CNRS/IN2P3, IJCLAB}, \orgaddress{\city{Orsay}, \postcode{91400}, \country{France}}}
\affil[8]{\orgname{INFN}, \orgdiv{Sezione di Roma Tor Vergata}, \orgaddress{\city{Rome}, \postcode{I-00133}, \country{Italy}}}
\affil[9]{\orgname{Jagiellonian University}, \orgaddress{\city{Kraków}, \postcode{31-007}, \country{Poland}}}
\affil[10]{\orgname{National Institute for Nuclear Physics}, \orgdiv{Catania}, \orgaddress{\city{Catania}, \postcode{95125}, \country{Italy}}}
\affil[11]{\orgname{Messiah University}, \orgaddress{\city{Mechanicsburg}, \postcode{17055}, \state{PA}, \country{US}}}
\affil[12]{\orgname{Laboratory Nuclear and High-Energy Physics}, \orgdiv{CNRS}, \orgaddress{\city{Paris}, \postcode{75005}, \country{France}}}
\affil[13]{\orgname{University of Manitoba}, \orgdiv{Physics}, \orgaddress{\city{Winnipeg}, \state{MB}, \postcode{R3T 2N2}, \country{Canada}}}
\affil[14]{\orgname{CERN}, \orgdiv{Accelerators and Beam Physics Group}, \orgaddress{\city{Geneva}, \postcode{CH-1211}, \country{Switzerland}}}
\affil[15]{\orgname{Oak Ridge National Laboratory}, \orgaddress{\city{Oak Ridge}, \state{TN}, \postcode{37830}, \country{USA}}}
\affil[16]{\orgname{Vanderbilt University}, \orgaddress{\city{Nashville}, \state{TN} , \postcode{37235}, \country{USA}}}
\affil[17]{\orgname{University of Virginia}, \orgaddress{\city{Charlottesville}, \state{VA}, \postcode{22904}, \country{USA}}}
\affil[18]{\orgname{Duke University}, \orgaddress{\city{Durham}, \state{NC}, \postcode{27708}, \country{USA}}}
\affil[19]{\orgname{University of Cincinnati}, \orgaddress{\city{Cincinnati}, \state{OH}, \postcode{45221}, \country{USA}}}
\affil[20]{\orgname{Fermilab}, \orgaddress{\city{Batavia}, \state{IL}, \postcode{60510}, \country{USA}}}
\affil[21]{\orgname{Lawrence Berkeley National Laboratory}, \orgaddress{\city{Berkeley}, \state{CA}, \postcode{94720}, \country{USA}}}
\affil[22]{\orgname{Argonne National Laboratory}, \orgaddress{\city{Lemont}, \state{IL}, \postcode{60439}, \country{USA}}}
\affil[23]{\orgname{Christopher Newport University}, \orgaddress{\city{Newport News}, \state{VA}, \postcode{23606}, \country{USA}}}
\affil[24]{\orgname{Rutgers University}, \orgaddress{\city{Camden}, \state{NJ}, \postcode{08102}, \country{USA}}}
\affil[25]{\orgname{University of Regina}, \orgaddress{\city{Regina}, \state{SK}, \postcode{S4S0A2}, \country{Canada}}}
\affil[26]{\orgname{Pacific Northwest National Laboratory}, \orgaddress{\city{Richland}, \state{WA}, \postcode{99354}, \country{USA}}}
\affil[27]{\orgname{University of California Irvine}, \orgaddress{\city{Irvine}, \state{CA}, \postcode{92697}, \country{USA}}}
\affil[28]{\orgname{Indian Institute of Technology Bombay}, \orgaddress{\city{Mumbai}, \state{Maharashtra}, \postcode{400076}, \country{India}}}
\affil[29]{\orgname{National Institute for Nuclear Physics}, \orgdiv{Genoa}, \orgaddress{\city{Genoa}, \postcode{I-16146}, \country{Italy}}}
\affil[30]{\orgname{Center for Frontiers in Nuclear Science, Stony Brook University}, \orgaddress{\city{Stony Brook}, \state{NY}, \postcode{11790-3800}, \country{USA}}}
\affil[31]{\orgname{National Institute for Nuclear Physics}, \orgdiv{Roma}, \orgaddress{\city{Rome}, \postcode{I-00185}, \country{Italy}}}
\affil[32]{\orgname{The Catholic University of America}, \orgaddress{\city{Washington}, \state{DC}, \postcode{20064}, \country{USA}}}
\affil[33]{\orgname{University of Glasgow}, \orgaddress{\city{Glasgow}, \postcode{G12 8QQ}, \country{United Kingdom}}}
\affil[34]{\orgname{Departamento de F\'isica Te\'orica \& IPARCOS, Universidad Complutense de Madrid}, \orgaddress{\city{ adrid}, \postcode{E-28040}, \country{Spain}}}
\affil[36]{\orgname{RIKEN BNL Research Center}, \orgaddress{\city{Upton}, \state{NY}, \postcode{11973}, \country{USA}}}
\affil[37]{\orgname{Institut f\"ur Theoretische Physik, Universit\"at Regensburg}, \orgaddress{\city{Regensburg}, \postcode{D-93040}, \country{Germany}}} 
\affil[35]{\orgname{Institute for Theoretical Physics, T\"{u}bingenUniversity}, \orgaddress{\city{T\"{u}bingen}, \postcode{72076}, \country{Germany}}}
\affil[38]{\orgname{Old Dominion University}, \orgaddress{\city{Norfolk}, \state{VA}, \postcode{23529}, \country{USA}}}
\affil[39]{\orgname{Center for Nuclear Femtography}, \orgaddress{\city{Washington DC}, \postcode{20005}, \country{USA}}}
\affil[40]{\orgname{University of Michigan}, \orgaddress{\city{Ann Arbor}, \state{MI}, \postcode{48104}, \country{USA}}}
\affil[41]{\orgname{Brookhaven National Laboratory}, \orgdiv{Department of Physics}, \orgaddress{\city{Upton, NY}, \postcode{11973-5000}, \country{USA}}}
\affil[42]{\orgname{Florida International University}, \orgaddress{\city{Miami}, \state{FL}, \postcode{33199},  \country{USA}}}
\affil[43]{\orgname{Rutgers University}, \orgaddress{\city{Piscataway}, \state{NJ}, \postcode{08854}, \country{USA}}}
\affil[44]{\orgname{Departamento de F\'isica Fundamental e IUFFyM, Universidad de Salamanca}, \orgaddress{\city{Salamanca}, \postcode{37008}, \country{Spain}}}
\affil[45]{\orgname{GFIMA - Escuela de Ciencias, Ingenier\'ia y Dise\~no, Universidad Europea de Valencia}, \orgaddress{\city{Valencia}, \postcode{46010}, \country{Spain}}}
\affil[46]{\orgname{University of Victoria}, \orgaddress{\city{Victoria}, \postcode{V8P 5C2}, \country{Canada}}}
\affil[47]{\orgname{National Centre For Nuclear Research}, \orgaddress{\city{Warsaw}, \postcode{02-093}, \country{Poland}}}
\affil[48]{\orgname{Future University in Egypt}, \orgaddress{\city{New Cairo}, \postcode{11835}, \country{Egypt}}}
\affil[49]{\orgname{Warsaw University of Technology}, \orgaddress{\city{Warsaw}, \state{}, \postcode{00-661}, \country{Poland}}}
\affil[50]{\orgname{University of California Los Angeles}, \orgaddress{\city{Los Angeles}, \state{CA}, \postcode{90095}, \country{USA}}}
\affil[51]{\orgname{Lawrence Livermore National Laboratory}, \orgaddress{\city{Livermore}, \state{CA}, \postcode{94550}, \country{USA}}}
\affil[52]{\orgname{Panjab University}, \orgaddress{\city{Chandigarh}, \postcode{PIN-160014}, \country{India}}}
\affil[53]{\orgname{University of York}, \orgaddress{\city{York}, \state{}, \postcode{YO422SF}, \country{United Kingdom}}}
\affil[54]{\orgname{Charles University, Faculty of Mathematics and Physics}, \orgaddress{\city{Prague}, \postcode{18000}, \country{Czech Republic}}}
\affil[55]{\orgname{Stony Brook University}, \orgaddress{\city{Stony Brook}, \state{NY}, \postcode{11794}, \country{USA}}}
\affil[56]{\orgname{Facultad de Ciencias F\'isico-Matem\'aticas, Universidad Aut\'onoma de Sinaloa, Ciudad Universitaria}, \city{Culiac\'an, Sinaloa} \postcode{80000}, \country{M\'exico}}
\affil[57]{\orgname{Hampton University}, \orgaddress{\city{Hampton}, \state{VA}, \postcode{23668}, \country{USA}}}
\affil[58]{\orgname{Nuclear Physics Division, Bhabha Atomic Research Centre}, \orgaddress{\city{Mumbai}, \postcode{400085}, \country{India}}}
\affil[59]{\orgname{Homi Bhabha National Institute}, \orgaddress{\city{Mumbai}, \postcode{400094}, \country{India}}}
\affil[60]{\orgname{Central University of Karnataka}, \orgaddress{\city{Kalaburagi}, \state{}, \postcode{585367}, \country{India}}}
\affil[61]{\orgname{Deggendorf Institute of Technology}, \orgaddress{\city{Deggendorf}, \postcode{94469}, \country{Germany}}}
\affil[62]{\orgname{Baruch College}, \orgaddress{\city{New York}, \state{NY}, \postcode{10010}, \country{USA}}}
\affil[63]{\orgname{Drexel University}, \orgaddress{\city{Philadelphia}, \state{PA}, \postcode{19104}, \country{US}}}
\affil[64]{\orgname{Center for Frontiers in Nuclear Science, Stony Brook University}, \orgdiv{Department of Physics and Astronomy}, \orgaddress{\city{Stony Brook}, \state{NY}, \postcode{11794}, \country{USA}}}

%\affil[63]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[64]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[65]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[66]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[67]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[68]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[69]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[70]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[71]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}
%\affil[72]{\orgname{University of }, \orgaddress{\city{City}, \state{}, \postcode{}, \country{Country}}}


==> authors/affiliations.tex <==
%
% Full ECCE author list
% Formatted for NIM

\affiliation[AANL]{organization={A. Alikhanyan National Laboratory},
	 city={Yerevan},
	 country={Armenia}} 
 
\affiliation[AcademiaSinica]{organization={Institute of Physics, Academia Sinica},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[AUGIE]{organization={Augustana University},
	 city={Sioux Falls},
	 state={SD},
	 country={USA}} 
	 
\affiliation[BGU]{organizatoin={Ben-Gurion University of the Negev}, 
      city={Beer-Sheva},
      country={Israel}}
      

 
\affiliation[BNL]{organization={Brookhaven National Laboratory},
	 city={Upton},
	 state={NY},
	 country={USA}} 
 
\affiliation[BrunelUniversity]{organization={Brunel University London},
	 city={Uxbridge},
	 country={UK}} 
 
\affiliation[CanisiusCollege]{organization={Canisius College},
	 city={Buffalo},
	 state={NY},
	 country={USA}} 
 
\affiliation[CCNU]{organization={Central China Normal University},
	 city={Wuhan},
	 country={China}} 
 
\affiliation[Charles]{organization={Charles University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[CIAE]{organization={China Institute of Atomic Energy, Fangshan},
	 city={Beijing},
	 country={China}} 
 
\affiliation[CNU]{organization={Christopher Newport University},
	 city={Newport News},
	 state={VA},
	 country={USA}} 
 
\affiliation[Columbia]{organization={Columbia University},
	 city={New York},
	 state={NY},
	 country={USA}} 
 
\affiliation[CUA]{organization={Catholic University of America},
	 city={Washington DC},
	 country={USA}} 
 
\affiliation[CzechTechUniv]{organization={Czech Technical University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[Duquesne]{organization={Duquesne University},
	 city={Pittsburgh},
	 state={PA},
	 country={USA}}  
 
\affiliation[FIU]{organization={Florida International University},
	 city={Miami},
	 state={FL},
	 country={USA}} 
 
\affiliation[GeorgiaState]{organization={Georgia State University},
	 city={Atlanta},
	 state={GA},
	 country={USA}} 
 
\affiliation[Glasgow]{organization={University of Glasgow},
	 city={Glasgow},
	 country={UK}} 
 
\affiliation[GSI]{organization={GSI Helmholtzzentrum fuer Schwerionenforschung GmbH},
	 city={Darmstadt},
	 country={Germany}} 
 
\affiliation[GWU]{organization={The George Washington University},
	 city={Washington, DC},
	 country={USA}} 
 

\affiliation[HUJI]{organization={Hebrew University},
	 city={Jerusalem},
	 country={Isreal}} 
 
\affiliation[IJCLabOrsay]{organization={Universite Paris-Saclay, CNRS/IN2P3, IJCLab},
	 city={Orsay},
	 country={France}} 
	 
\affiliation[CEA]{organization={IRFU, CEA, Universite Paris-Saclay},
     cite= {Gif-sur-Yvette},
     country={France}
}


\affiliation[IMP]{organization={Chinese Academy of Sciences},
	 city={Lanzhou},
	 country={China}} 
 
\affiliation[IowaState]{organization={Iowa State University},
	 city={Iowa City},
	 state={IA},
	 country={USA}} 
 
\affiliation[JazanUniversity]{organization={Jazan University},
	 city={Jazan},
	 country={Sadui Arabia}} 
 
\affiliation[JLab]{organization={Thomas Jefferson National Accelerator Facility},
	 city={Newport News},
	 state={VA},
	 country={USA}} 

 
\affiliation[KobeUniversity]{organization={Kobe University},
	 city={Kobe},
	 country={Japan}} 
 
\affiliation[Kyungpook]{organization={Kyungpook National University},
	 city={Daegu},
	 country={Republic of Korea}} 
 
\affiliation[LANL]{organization={Los Alamos National Laboratory},
	 city={Los Alamos},
	 state={NM},
	 country={USA}} 
 
\affiliation[LehighUniversity]{organization={Lehigh University},
	 city={Bethlehem},
	 state={PA},
	 country={USA}} 
 
\affiliation[LLNL]{organization={Lawrence Livermore National Laboratory},
	 city={Livermore},
	 state={CA},
	 country={USA}} 
 
\affiliation[MoreheadState]{organization={Morehead State University},
	 city={Morehead},
	 state={KY},
	 }
 
\affiliation[MIT]{organization={Massachusetts Institute of Technology},
	 city={Cambridge},
	 state={MA},
	 country={USA}} 
 
\affiliation[MSU]{organization={Mississippi State University},
	 city={Mississippi State},
	 state={MS},
	 country={USA}} 
 
\affiliation[NCKU]{organization={National Cheng Kung University},
	 city={Tainan},
	 country={Taiwan}} 
 
\affiliation[NCU]{organization={National Central University},
	 city={Chungli},
	 country={Taiwan}} 
 
\affiliation[Nihon]{organization={Nihon University},
	 city={Tokyo},
	 country={Japan}} 
 
\affiliation[NMSU]{organization={New Mexico State University},
	 city={Las Cruces},
	 state={NM},
	 country={USA}} 
 
\affiliation[NRNUMEPhI]{organization={National Research Nuclear University MEPhI},
	 city={Moscow},
	 country={Russian Federation}} 
 
\affiliation[NRCN]{organization={Nuclear Research Center - Negev},
	 city={Beer-Sheva},
	 country={Isreal}} 
 
\affiliation[NTHU]{organization={National Tsing Hua University},
	 city={Hsinchu},
	 country={Taiwan}} 
 
\affiliation[NTU]{organization={National Taiwan University},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[ODU]{organization={Old Dominion University},
	 city={Norfolk},
	 state={VA},
	 country={USA}} 
 
\affiliation[Ohio]{organization={Ohio University},
	 city={Athens},
	 state={OH},
	 country={USA}} 
 
\affiliation[ORNL]{organization={Oak Ridge National Laboratory},
	 city={Oak Ridge},
	 state={TN},
	 country={USA}} 
 
\affiliation[PNNL]{organization={Pacific Northwest National Laboratory},
	 city={Richland},
	 state={WA},
	 country={USA}} 
 
\affiliation[Pusan]{organization={Pusan National University},
	 city={Busan},
	 country={Republic of Korea}} 
 
\affiliation[Rice]{organization={Rice University},
	 city={Houston},
	 state={TX},
	 country={USA}} 
 
\affiliation[RIKEN]{organization={RIKEN Nishina Center},
	 city={Wako},
	 state={Saitama},
	 country={Japan}} 
 
\affiliation[Rutgers]{organization={The State University of New Jersey},
	 city={Piscataway},
	 state={NJ},
	 country={USA}} 
 
 
\affiliation[CFNS]{organization={Center for Frontiers in Nuclear Science},
	 city={Stony Brook},
	 state={NY},
	 country={USA}} 
 
\affiliation[StonyBrook]{organization={Stony Brook University},
	 city={Stony Brook},
	 state={NY},
	 country={USA}} 
 
\affiliation[RBRC]{organization={RIKEN BNL Research Center},
	 city={Upton},
	 state={NY},
	 country={USA}} 
	 
\affiliation[SDU]{organizaton={Shandong University},
     city={Qingdao},
     state={Shandong},
     country={China}}
     
\affiliation[Seoul]{organization={Seoul National University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[Sejong]{organization={Sejong University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[Shinshu]{organization={Shinshu University},
         city={Matsumoto},
	 state={Nagano},
	 country={Japan}} 
 
\affiliation[Sungkyunkwan]{organization={Sungkyunkwan University},
	 city={Suwon},
	 country={Republic of Korea}} 
 
\affiliation[TAU]{organization={Tel Aviv University},
	 city={Tel Aviv},
	 country={Israel}} 

\affiliation[USTC]{organization={University of Science and Technology of China},
     city={Hefei},
     country={China}}

\affiliation[Tsinghua]{organization={Tsinghua University},
	 city={Beijing},
	 country={China}} 
 
\affiliation[Tsukuba]{organization={Tsukuba University of Technology},
	 city={Tsukuba},
	 state={Ibaraki},
	 country={Japan}} 
 
\affiliation[CUBoulder]{organization={University of Colorado Boulder},
	 city={Boulder},
	 state={CO},
	 country={USA}} 
 
\affiliation[UConn]{organization={University of Connecticut},
	 city={Storrs},
	 state={CT},
	 country={USA}} 
 
\affiliation[UNGeorgia]{organization={University of North Georgia},
     cite={Dahlonega}, 
     state={GA},
     country={USA}}
     
\affiliation[UH]{organization={University of Houston},
	 city={Houston},
	 state={TX},
	 country={USA}} 
 
\affiliation[UIUC]{organization={University of Illinois}, 
	 city={Urbana},
	 state={IL},
	 country={USA}} 
 
\affiliation[UKansas]{organization={Unviersity of Kansas},
	 city={Lawrence},
	 state={KS},
	 country={USA}} 
 
\affiliation[UKY]{organization={University of Kentucky},
	 city={Lexington},
	 state={KY},
	 country={USA}} 
 
\affiliation[Ljubljana]{organization={University of Ljubljana, Ljubljana, Slovenia},
	 city={Ljubljana},
	 country={Slovenia}} 
 
\affiliation[NewHampshire]{organization={University of New Hampshire},
	 city={Durham},
	 state={NH},
	 country={USA}} 
 
\affiliation[Oslo]{organization={University of Oslo},
	 city={Oslo},
	 country={Norway}} 
 
\affiliation[Regina]{organization={ University of Regina},
	 city={Regina},
	 state={SK},
	 country={Canada}} 
 
\affiliation[USeoul]{organization={University of Seoul},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[UTsukuba]{organization={University of Tsukuba},
	 city={Tsukuba},
	 country={Japan}} 
	 
\affiliation[UoT]{organization={University of Texas},
    city={Austin},
    state={Texas},
    country={USA}}
 
\affiliation[UTK]{organization={University of Tennessee},
	 city={Knoxville},
	 state={TN},
	 country={USA}} 
 
\affiliation[UVA]{organization={University of Virginia},
	 city={Charlottesville},
	 state={VA},
	 country={USA}} 
 
\affiliation[Vanderbilt]{organization={Vanderbilt University},
	 city={Nashville},
	 state={TN},
	 country={USA}} 

\affiliation[VirginiaUnion]{organization={Virginia Union University},
	 city={Richmond},
	 state={VA},
	 country={USA}} 
 
\affiliation[WayneState]{organization={Wayne State University},
	 city={Detroit},
	 state={MI},
	 country={USA}} 
 
\affiliation[WI]{organization={Weizmann Institute of Science},
	 city={Rehovot},
	 country={Israel}} 
 
\affiliation[WandM]{organization={The College of William and Mary},
	 city={Williamsburg},
	 state={VA},
	 country={USA}} 
 
\affiliation[Yamagata]{organization={Yamagata University},
	 city={Yamagata},
	 country={Japan}} 
 
\affiliation[Yarmouk]{organization={Yarmouk University},
	 city={Irbid},
	 country={Jordan}} 
 
\affiliation[Yonsei]{organization={Yonsei University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[York]{organization={University of York},
	 city={York},
	 country={UK}} 


==> authors/authors-alphabetical.tex <==
%
% Full list of ECCE Collaboratotions
%
% Click Refresh to get the latest version
%
% Goto the following to edit:
% https://www.overleaf.com/1234763137gmqgnzsrpsdj
%

\author[MIT,WandM,JLab]{C.~Fanelli}
\author[Regina]{Z.~Papandreou}
\author[Regina]{K.~Suresh}
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN,RBRC]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[MSU]{C. Ayerbe Gayoso}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[BNL,JLab]{M.D.~Baker}
\author[York]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CUA]{V.~Berdnikov}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier~\corref{cor1}}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[CUA]{J.~Crafts}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'e}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
%\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[York]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[MIT,JLab]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL,UTK]{E.~Glimos}
\author[RIKEN,RBRC]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[CUA]{T.~Horn}
\author[AANL]{A.~Hoghmrtsyan}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yonsei]{K.~Y.~Hwang}
\author[ODU]{C.~E.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[CUA]{G.~Kalicy}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~J.~D.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Sungkyunkwan]{H.~Lee}
\author[USeoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.B.~Li}
\author[USTC]{X.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[MIT]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-H.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[York]{W.~Lynch}
\author[UNGeorgia]{S.~Mantry}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[UoT]{C.~Markert}
\author[FIU]{P.~Markowitz}
\author[AANL]{H.~Marukyan}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[AANL]{A.~Mkrtchyan}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[AANL]{A.~Movsisyan}
\author[AANL]{H.~Mkrtchyan}
\author[AANL]{A.~Mkrtchyan}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v si\'c}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
%\author[Regina]{Z.~Papandreou}
\author[NMSU]{S.~F.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~L.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL,UTK]{K.F.~Read}
\author[Oslo]{K.~R\o ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN,RBRC]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[Glasgow,CEA]{D.~Sokhan}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[CUA]{P.~Stepanov}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
%\author[Regina]{K.~Suresh}
\author[AANL]{V.~Tadevosyan}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UoT]{D.~Thomas}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[CUA]{R.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[IJCLabOrsay]{C.~Van~Hulse}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[York]{D.~P.~Watts}
\author[CUA]{N.~Wickramaarachchi}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yonsei]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[York]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[USTC]{W.~Zha}
\author[SDU]{J.-L.~Zhang}
\author[UVA]{J.-X.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.-X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


\cortext[cor1]{Deceased}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


